Evading classifiers in discrete domains with provable optimality guarantees

Machine-learning models for security-critical applications such as bot, malware, or spam detection, operate in constrained discrete domains. These applications would benefit from having provable guarantees against adversarial examples. The existing literature on provable adversarial robustness of models, however, exclusively focuses on robustness to gradient-based attacks in domains such as images. These attacks model the adversarial cost, e.g., amount of distortion applied to an image, as a $p$-norm. We argue that this approach is not well-suited to model adversarial costs in constrained domains where not all examples are feasible. We introduce a graphical framework that (1) generalizes existing attacks in discrete domains, (2) can accommodate complex cost functions beyond $p$-norms, including financial cost incurred when attacking a classifier, and (3) efficiently produces valid adversarial examples with guarantees of minimal adversarial cost. These guarantees directly translate into a notion of adversarial robustness that takes into account domain constraints and the adversary's capabilities. We show how our framework can be used to evaluate security by crafting adversarial examples that evade a Twitter-bot detection classifier with provably minimal number of changes; and to build privacy defenses by crafting adversarial examples that evade a privacy-invasive website-fingerprinting classifier.

==> parts/bfs.tex <==
\section{Instantiations of attacks in discrete domains as best-first search}%
\label{app:related-instantiations}

\subsection{Best-first search algorithms}
In Algorithm~\ref{alg:bfs} we show the pseudocode of a variant of generalized best-first search
called BF$^*$~\cite{DechterP85}. Several common search algorithms, like uniform-cost search, greedy
best-first search, and \astar variants, are specializations of BF$^*$. They differ in their
instantiation of the scoring function used to select the best nodes at each step of the algorithm.
Additionally, by limiting the number of items in data structure holding candidate nodes, one can obtain
best-first beam search and hill climbing algorithms~\cite{RichKnight91}. We summarize these differences
in~\Tabref{tab:search-algos}.

\begin{algorithm*}[t]
\caption{BF$^*$ search algorithm}\label{alg:bfs}
  \begin{algorithmic}[1]
	\Require{Priority queue data structure $\opensetstruct$}
	\Require{Directed graph $\gG = (V, E)$}
	\Require{Scoring function $\scorefunc: V \times V \rightarrow \sR$}
	\Require{Goal predicate $\isgoal: V \rightarrow \{0, 1\}$}
	\Require{Starting node $s \in V$}
    \Function{BF$^*$}{$\gG$, $\scorefunc(\cdot)$, $\isgoal(\cdot)$; $s$}
        \Let{\openset}{$\opensetstruct(\{s\})$}
		\Let{\closedset}{$\{\}$}
		\While{\openset is not empty}
			\Let{$v$}{remove node from \openset with the lowest recorded value of $f$-score}
			\If{$\isgoal(v)$}
				\Return $v$
			\EndIf
			\Let{\closedset}{$\closedset \cup \{v\}$}
			\For{each child $v'$ of $v$ in $\gG$}
				\Let{$\scorefunc$-value}{$\scorefunc(v, v')$}
				\If{$v'$ \emph{not} in \openset or \closedset}
					\State{Record $v'$ into \openset with $\scorefunc$-value}
				\EndIf
				\If{$v'$ is in \openset or \closedset and $\scorefunc$-value is lower than recorded}
					\State{Replace $v'$ with the updated $\scorefunc$-value in the respective set}
					\If{$v'$ is in \closedset}
						\State{Move $v'$ to \openset}
					\EndIf
				\EndIf
			\EndFor
		\EndWhile
    \EndFunction
  \end{algorithmic}
\end{algorithm*}


\begin{table}[t]
    \centering
    \caption{Specializations of BF$^*$}\label{tab:search-algos}
    \begin{tabular}{ll}
        \toprule
        \textbf{Algorithm} & \textbf{$\scorefunc$} \\
        \midrule
        Greedy best-first~\cite{DoranMichie66}
        & $h(v')$
        \\

        Uniform-cost~\cite{HartNR68}
        & $\edgecost(v, v')$
        \\

        \astar~\cite{HartNR68}
        & $\edgecost(v, v') + h(v')$
        \\

        $\varepsilon$-weighted \astar~\cite{Pohl70}
        & $\edgecost(v, v') + \varepsilon h(v')$
        \\

        \bottomrule

        \\

        \toprule
        \textbf{Algorithm} & \textbf{$\opensetstruct$} \\
        \midrule
        Hill climbing
        & Limited to one highest-scoring item
        \\

        Best-first beam search~\cite{RichKnight91}
        & Limited to $B$ highest-scoring items
        \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{Instantiations}
We can use the graphical framework formalization, described in \Secref{sec:model}, to instantiate
several existing attacks against machine learning classifiers in discrete domains.
\Tabref{tab:comparison} outlines the instantiations of these attacks as applications of best-first
search over a transformation graph. The attacks differ in their general setting, transformation
graphs, and the scoring function choice. Note that for all cases, each child in a transformation
graph (column \emph{expansions} in the table) represents a single atomic transformation.
Transformations thus compound with the depth of the traversal of the graph. For those attacks that
can be instantiated as greedy search, if \emph{cost} is shown, it is enforced by truncating the
transformation graph once a certain cost threshold is reached.

\begin{sidewaystable*}
    \input{parts/extras/pretty_comparison.tex}
\end{sidewaystable*}


==> parts/eval-credit.tex <==
To extensively evaluate the minimal-cost attack using heuristic graph search against non-informed
(breadth-first) search, we choose a problem with a small branching factor of the transformation
graph. This allows the breadth-first search to finish within reasonable time.

For this, we consider an application to fraud detection using UCI~\cite{uciml} German credit risk
dataset. The dataset contains 1000 feature vectors representing loan applications along with the
details about the applicant. Each example has a binary label encoding whether the person has
defaulted on the loan or not.

The features include job type, housing type, income bracket, loan amount, loan duration, loan
purpose, etc. \bknote{TODO: Rewrite this paragraph, see bots for an example} Following a common
practice when using linear models, we quantize all the continuous features (e.g., income bracket).
The number of bins used for quantization allows us to control the size of the transformation graph:
the more bins the larger the graph.

We one-hot encode the quantized and categorical features. Then, we train a regularized logistic
regression classifier to predict the probability of a person defaulting on a loan. We split the
dataset into 900 train examples and 100 test examples, and fit the model using 5-fold stratified
cross-validation on the train dataset. The results vary slightly depending on the 

\bknote{TODO: Report performance with different quantization levels}

% Our model achieves 71\% accuracy on the test dataset (72\% precision, 93\% recall).
\descr{Transformation graph}
We assume that all features that represent information about a person are constant. We only modify
loan duration, loan amount, and loan purpose, since these features are arguably easy to modify in a
realistic setting (changing the loan application form). Starting with a given initial example $x$,
we define the direct descendants as vectors $x'_i$, each of which change one of the following:
\begin{itemize}
    \item The current loan amount bin into a bin immediately higher or lower. This
        results in up to 2 transformed examples for each parent example.
    \item The current loan duration into a bin immediately higher or lower. This results in up to 2
        transformed examples at each parent example.
    \item The current loan purpose category into any other purpose category.  This results in up to
        7 transformed examples (since there are 8 possible categories) for each parent example.
\end{itemize}
We set the cost of each transformation to $\lp[1]$ distance between feature vectors. Each of them is
always 2 in our case, since exactly two bits are different between transformations.

\descr{Modeling adversarial cost}
\bknote{TODO: Explain relationship of path costs to the real cost}

\descr{Search efficiency}
\bknote{TODO: Update figures}
For each example in the full dataset we run the breadth-first search (BFS) on the graph and \astar
using the heuristic $\hinputspace$, until we find the first modification of the example that changes
the decision of the classifier. The BFS serves as the baseline. For \astar, we also run different
$\varepsilon$-relaxations (see \Secref{sec:attack-relaxations}). We present the results in
Fig.~\ref{fig:a_star_bfs_comparison}. For those examples that don't require many changes, both
\astar and BFS traverse similarly-sized parts of the graph. When the number of nodes that need to be
traversed gets larger, the relative improvement of the \astar becomes more prominent, reaching up to
140\% in some cases.

\descr{Provable guarantees}
We show in Fig.~\ref{fig:adv_costs} the distribution of the number of changes in the produced adversarial
examples. Since each transformation has the $\lp[1]$ cost of 2, we divide the resulting costs by 2
to only show the number of changes itself. For this particular model and the dataset, the attacker
only needs to apply one change to most of the examples to flip the decision of the classifier. This
means the classifier is likely not robust to adversarial manipulation.

\begin{figure}
\centering
\caption{Comparison of performance of \astar vs BFS. The first graph shows the number of expanded
    nodes during search on a logarithmic scale. The second graph shows the relative improvement in
    number of expansions of \astar relative to BFS.}
\label{fig:a_star_bfs_comparison}
\end{figure}

\begin{figure}
\centering
\caption{Cost distribution of the found adversarial examples}
\label{fig:adv_costs}
\end{figure}



==> parts/extras/comparison.tex <==
\caption{Instantiations of existing attacks within the graphical framework}%
\label{tab:comparison}
\scalebox{0.9}{%
    \begin{tabular}{l|p{1.5cm}|p{1.7cm}p{4cm}p{2.5cm}p{4cm}p{4cm}p{2cm}}
        Attack & Domain & Adversary knowledge & Expansions & Cost & Heuristic & Scoring function /
        Search algorithm & Admissibility \\
    \toprule
    \citet{PapernotMSH16}
    & Text
    & White-box
    & Substitutions of a word with any other word in the vocabulary
    & Number of substitutions
    & Forward gradient-based
    & Heuristic
    / Hill climbing
    & \nope \\

    \citet{textfool}
    & Text
    & White-box
    & Word synonym substitutions; character substitutions, insertions, deletions
    & Semantic dissimilarity
    & Forward gradient-based
    & Non-linear combination of cost and heuristic
    / Best-first
    & \nope \\

    \citet{LiangSBLS18}
    & Text
    & White-box
    & Insertion of common phrases, word removal, character substitution and homoglyph insertions
    & ---
    & Forward gradient-based
    & Heuristic
    / Greedy best-first
    & \nope \\

    \citet{EbrahimiRLD18}
    & Text
    & White-box
    & Character/word substitution, insertion, deletion
    & ---
    & Forward gradient-based
    & Heuristic
    / Best-first beam search
    & \nope \\

    \citet{GaoLSQ18}
    & Text
    & Black-box
    & Character substitution, insertion, deletion
    & ---
    & Confidence-based
    & Heuristic
    / Hill climbing
    & \nope \\

    \midrule

    \citet{GrossePM0M16}
    & Malware
    & White-box
    & Bit flips
    & $\lp$
    & Forward gradient-based
    & Heuristic
    / Hill climbing
    & \nope \\

    \midrule

    \citet{JiaG18}
    & {\footnotesize App recom\-men\-dations}
    & White-box
    & Item addition, modification
    & $\lp$
    & Forward gradient-based
    & Heuristic
    / Hill climbing
    & \nope \\

    \midrule
    \citet{OverdorfKBTG18}
    & Credit scoring
    & Black-box
    & Category modifications
    & Number of modifications
    & ---
    & Cost
    / Uniform-cost search
    & \yup \\

    \midrule
    Ours
    & *
    & White-box
    & *
    & Graph path cost, with $\lp$ edge costs
    & Lower bound on minimal adversarial cost over continuous domain
    & Linear combination of cost and heuristic
    / \astar
    & \yup \\

\end{tabular}
}{}


==> parts/heuristic.tex <==
\section{Improving the heuristic in the optimal instantiation}

In the previous section we have presented a setting and a heuristic which allows to a find
minimal-cost adversarial examples using \astar search. We now show how to construct heuristics that
improve on the heuristic constructed from the exact value of adversarial robustness $\dist(x)$ by
incorporating knowledge about the transformation graph.

\subsection{Feature space constraints for linear models}
In practice, only a part of the full feature vector may be transformable. In our running example,
imagine if the adversary could not change the \emph{days since the account was created} feature out
of practicality constraints. In such case, the heuristic value can be improved by taking these
constraints into account. We show how to do this for linear models, i.e., with $\phi(\vx) = \vx$.

Let $\proj{J}(\vx)$ denote a projection of a vector $\vx \in \sX \subset \sR^m$:
\[\proj{J}(\vx) = [x_j]_{j \in J}\]
for a set of indices $J \subset \{1, 2, ..., m\}^k$, with $k < m$. The set $J$ represents the set of
feature indices that can be transformed in the transformation graph $\gG$.
% We denote by $\bar J$ the set of all other indices that can not be
% transformed: $\bar J = \{1, 2, ..., m\} \setminus J$.

Then, we can re-define the original discriminant function $f: \sR^m \rightarrow \{0, 1\}$ in terms
of the projected inputs as follows:
\[
    f^\downarrow(\vx) = \underbrace{(\proj{J}(\vw)) \cdot (\proj{J}(\vx))}_{\vw^\downarrow \cdot
    \proj{J}(\vx)} + \underbrace{(\proj{\bar J}(\vw)) \cdot (\proj{\bar J}(\vx)) + b}_{b^\downarrow}
\]
Since only features $J$ vary for all transformations in the graph $\gG = (V, E, \edgecost)$,
$f^\downarrow$ is an equivalent re-parametrization:
\[
    f^\downarrow(\vx) = f(\vx) \quad \text{for all $\vx \in V$}
\]

Note that the values $\vw^\downarrow$, $b^\downarrow$ are fixed for all transformations.

Treating $f^\downarrow(\vx)$ as the target function, we can take into account the constraints:
\begin{equation}
    \dist^\downarrow(\vx) = \frac{|f^\downarrow(\vx)|}{\norm{\vw^\downarrow}_q}
\end{equation}

One can obtain an equivalent result by taking a partial gradient $\nabla_{\proj{J} \vx}f(\vx)$
in the Taylor expansion from \Eqref{eq:dist-nonlinear-decision-boundary}.

\subsection{Incorporating the knowledge about costs}
We now show two simple improvements of the basic heuristic that take into account the cost
distribution.

\descr{Minimal edge cost} Let the minimal possible cost of any edge in graph $\gG$ be $\theta$.
Then, we can define $\dist^\textsf{min}(x)$ as follows:
\[\dist^\textsf{min}(x) = \max(\theta, \dist(x))\]

\begin{statement}
    Let the transformation graph $\gG = (V, E, \edgecost)$ have $\edgecost(a, b) = \lp(a, b) \geq
    \theta$, and the initial example be $x \in V$. Then the heuristic defined by
    $\dist^\textsf{min}(x)$ is an admissible heuristic for the graph search problem from
    \Eqref{eq:mincost-graph-problem}.
\end{statement}
\begin{IEEEproof}
    By \Stmtref{thm:admissibility} and \Defref{def:admissibility}.
\end{IEEEproof}

\descr{Constant edge cost} In an extension of the previous case, assume that the cost of \emph{all}
edges is constant and is equal to $\sigma$. We can define $\dist^\textsf{grid}(x)$ as rounding of the
value of $\dist(x)$ up to the next multiple of $\sigma$:
\[\dist^\textsf{grid}(x) = \sigma \ceil{\frac{\dist(x)}{\sigma}}\]

\begin{statement}
    Let the transformation graph $\gG = (V, E, \edgecost)$ have $\edgecost(a, b) = \lp(a, b) =
    \sigma$ for all $a, b \in V$, and the initial example be $x \in V$. Then the heuristic defined
    by $\dist^\textsf{grid}(x)$ is an admissible heuristic for the graph search problem from
    \Eqref{eq:mincost-graph-problem}.
\end{statement}
\begin{IEEEproof}
    \bknote{TODO}
\end{IEEEproof}

We evaluate this heuristic in \Secref{sec:eval-bots}.


==> parts/non-optim-attack.tex <==
\section{Graph search approach}
\label{sec:non-optim-attack}

As detailed before, there exist numerous attacks that produce adversarial examples in various
discrete domains.  The majority of these attacks are based on greedy heuristic algorithms. Our
formalization of adversary's capabilities through a transformation graph (\Secref{sec:model}) allows
to view the problem of finding adversarial examples in discrete domains as graph search. This view
subsumes many of these attack techniques, and offers some additional benefits. In this section we
present some background on graph search algorithms and show how mentioned attacks can be formulated
as instances of graph search.

% We have presented the method to efficiently find adversarial examples in constrained discrete
% domains that are provably minimal-cost, or are provably within a multiplicative bound from the
% minimal cost. The method, however, can only be applied in certain settings. Nevertheless, the
% graphical framework is also useful for mounting attacks against ML without optimality guarantees. In
% this section we discuss how to do this.

\subsection{Best-first search algorithms}
\label{sec:bfs}

In Algorithm~\ref{alg:bfs} we show the pseudocode of a variant of generalized best-first search
called BF$^*$~\cite{DechterP85}. Uniform-cost search, greedy best-first search, and \astar variants,
are specializations of BF$^*$. They differ in their instantiation of the scoring function used to
select the best nodes at each step of the algorithm.  Additionally, by limiting the number of items
in data structure holding candidate nodes, one can obtain best-first beam search and hill climbing
algorithms~\cite{RichKnight91}. We summarize these differences in~\Tabref{tab:search-algos}.

\begin{algorithm}[t]
\caption{BF$^*$ search algorithm}\label{alg:bfs}
  \begin{algorithmic}[1]
	\Require{Priority queue data structure $\opensetstruct$}
	\Require{Directed graph $\gG = (V, E)$}
	\Require{Scoring function $\scorefunc: V \times V \rightarrow \sR$}
	\Require{Goal predicate $\isgoal: V \rightarrow \{0, 1\}$}
	\Require{Starting node $s \in V$}
    \Function{BF$^*$}{$\gG$, $\scorefunc(\cdot)$, $\isgoal(\cdot)$; $s$}
        \Let{\openset}{$\opensetstruct(\{s\})$}
		\Let{\closedset}{$\{\}$}
		\While{\openset is not empty}
			\Let{$v$}{remove node with lowest $f$-score from \openset}
			\If{$\isgoal(v)$}
				\Return $v$
			\EndIf
			\Let{\closedset}{$\closedset \cup \{v\}$}
			\For{each child $v'$ of $v$ in $\gG$}
				\Let{$\scorefunc$-value}{$\scorefunc(v, v')$}
				\If{$v'$ \emph{not} in \openset or \closedset}
					\State{Record $v'$ into \openset with $\scorefunc$-value}
				\EndIf
				\If{$v'$ is in \openset or \closedset and $\scorefunc$-value
                    \phantom{\hspace{5.2em}} is lower than recorded}
					\State{Replace $v'$ with the updated}
                    \State{\quad $\scorefunc$-value in the respective set}
					\If{$v'$ is in \closedset}
						\State{Move $v'$ to \openset}
					\EndIf
				\EndIf
			\EndFor
		\EndWhile
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\begin{table}[t]
    \centering
    \caption{Specializations of BF$^*$}\label{tab:search-algos}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ll}
        \toprule
        \textbf{Algorithm} & \textbf{$\scorefunc$} \\
        \midrule
        Greedy best-first~\cite{DoranMichie66}
        & $h(v')$
        \\

        Uniform-cost~\cite{HartNR68}
        & $\edgecost(v, v')$
        \\

        \astar~\cite{HartNR68}
        & $\edgecost(v, v') + h(v')$
        \\

        $\varepsilon$-weighted \astar~\cite{Pohl70}
        & $\edgecost(v, v') + \varepsilon h(v')$
        \\

        \bottomrule

        \\

        \toprule
        \textbf{Algorithm} & \textbf{$\opensetstruct$} \\
        \midrule
        Hill climbing
        & Limited to one best-scoring item
        \\

        Best-first beam search~\cite{RichKnight91}
        & Limited to $B$ best-scoring items
        \\
        \bottomrule
    \end{tabular}
    }
\end{table}

\subsection{Instantiations of existing attacks}
\label{sec:related-instantiations}

We can use the graphical framework formalization from in \Secref{sec:model}, to instantiate
several existing attacks against machine learning classifiers in discrete domains.
\Tabref{tab:comparison} outlines the instantiations of these attacks as applications of best-first
search over a transformation graph. The attacks differ in their general setting, transformation
graphs, and the scoring function choice. Note that for all cases, each child in a transformation
graph (column \emph{expansions} in the table) represents a single atomic transformation.
Transformations thus compound with the depth of the traversal of the graph. For those attacks that
can be instantiated as greedy search, if \emph{cost} is shown, it is enforced by truncating the
transformation graph once a certain cost threshold is reached.

Most of the attacks amount to running a hill climbing search algorithm over some \emph{implicit}
transformation graph. \citet{EbrahimiRLD18} take a step forward, and run beam search.
\citet{OverdorfKBTG18} use an exhaustive search over the space of feasible transformations,
equivalent to uniform-cost search.

\begin{sidewaystable}
    \input{parts/extras/pretty_comparison.tex}
\end{sidewaystable}

\medskip

% To demonstrate the advantages of the graphical framework, in \Secref{sec:eval-wfp} we use the
% best-first graph search algorithm to run attacks against network traffic classifier. This
% application shows that existing approaches to finding adversarial examples in discrete
% domains---almost always using hill climbing---can be improved by using other graph search
% algorithms. Even more, in the next section, \Secref{sec:optim-attack}, we show how in some settings
% one can leverage the graphical framework to obtain adversarial examples with provable optimality
% guarantees using \astar graph search.

In \Secref{sec:eval-wfp} we use the best-first graph search algorithm to run attacks against network
traffic classifier. To demonstrate an advantage of the graphical framework, in the next section,
\Secref{sec:optim-attack}, we show how in some settings one can leverage the framework to obtain
adversarial examples with provable optimality guarantees using \astar search.

